An anisotropic cohesive fracture model: advantages and limitations of length-scale insensitive phase-field damage models

The goal of the current work is to explore direction-dependent damage initiation and propagation within an arbitrary anisotropic solid. In particular, we aim at developing anisotropic cohesive phase-field (PF) damage models by extending the idea introduced in \cite{REZAEI2021a} for direction-dependent fracture energy and also anisotropic PF damage models based on structural tensors. The cohesive PF damage formulation used in the current contribution is motivated by the works of \cite{LORENTZ201120, wu2018, GEELEN2019}. The results of the latter models are shown to be insensitive with respect to the length scale parameter for the isotropic case. This is because they manage to formulate the fracture energy as a function of diffuse displacement jumps in the localized damaged zone. In the present paper, we discuss numerical examples and details on finite element implementations where the fracture energy, as well as the material strength, are introduced as an arbitrary function of the crack direction. Using the current formulation for anisotropic cohesive fracture, the obtained results are almost insensitive with respect to the length scale parameter. The latter is achieved by including the direction-dependent strength of the material in addition to its fracture energy. Utilizing the current formulation, one can increase the mesh size which reduces the computational time significantly without any severe change in the predicted crack path and overall obtained load-displacement curves. We also argue that these models still lack to capture mode-dependent fracture properties. Open issues and possible remedies for future developments are finally discussed as well.

==> arbit.tex <==
$c_0=\pi$

$\omega(d)= 2d - d^2$

$f_D = \dfrac{(1-d)^2}{(1-d)^2+a_1d+a_1a_2d^2}$

$H=\max_t (\psi_e^0(t),\psi_{th})$





$ \psi_c(d,\nabla d) = \psi_{c,s} = G_{c,0}~\gamma_s(d,\nabla d) $ 
$\psi_{c,a} = G_c(\theta)~\gamma_a(d,\nabla d)$ 


$\gamma_s(d,\nabla d)= \dfrac{1}{c_0 l_c}~\omega(d)~+~\dfrac{l_c}{c_0}~\nabla d \cdot \bm{A} \cdot \nabla d.$

$\gamma_a(d,\nabla d)= \dfrac{1}{c_ol_c}~\omega(d)~+~\dfrac{l_c}{c_0}~\nabla d \cdot \nabla d.$

$G_c(\theta) &= \sum_m \kappa_m\left(1+\alpha_m~\sin^2\left(m(\theta+\theta'_m \right))\right)$




$\psi_{th,a}=\dfrac{1}{2E}~\sigma_{u}^2(\theta)$

$\sigma_{u}(\theta) = \sum_m \sigma_{0,m}\left(1+\alpha_{m}~\sin^2\left(m(\theta+\theta'_{m} \right))\right)^{p_m}$

$\psi_{th,s} = \dfrac{1}{2}E~\varepsilon^2_0 = \dfrac{1}{2E}\sigma_0^2$

==> draft.tex <==
There is vast amount of developments and investigation to properly understand the mechanism of damage and fracture. Such understanding leads to accurate and effective nmerical models which serve to predict the materil behavior.

Yang et al. \cite{YANG2014349} presented a model which couples lithium diffusion with elasto-plastic deformation and can predict anisotropic swelling of lithiated material. 

 and argue that intermittent cracking may be understood as being due to a time lag in the diffusion of hydrogen towards the cohesive zone, since a buildup of hydrogen is necessary in order for the crack to advance.
 
 Failure mechanics and fracture modeling play a prominent role for predicting the collapse of structures and every other mechanical system during its usage time.
 
 %%%%%%%%%%% CDM
Early works on continuum damage models~(CDM)~ pioneered in~\cite{Kachanov1958} focus on modeling the macroscopic crack by considering local damage constitutive relations. These models are known to be meshed dependent see~\cite{Bazant1984}.
This leads to the non-local constitutive relations \cite{Drugan1996,etde_529023}. Defining the non-local variable as a weighted average of the corresponding value in the finite neighborhood which is defined by an internal length scale parameter see ~\cite{bazant87,peerlings1996}.
\textcolor{red}{We should ask Tim to modify the last paragraph.}

%The CZ model is extended widely in order to predict the fracture even in hard coatings see ~\cite{REZAEI201762} and even recently with considering non-local tractions~\cite{ortiz1999,REZAEI2020}.

% The energy-based criterion for damage, by which gradient extended damage models and phase-field damage models work, could result in damage occurrence in compression zones; therefore, an additive decomposition is crucial to split the strain tensor into a positive and negative parts see~\cite{AMOR2009,BORDEN2012}.

In the standard phase-field damage models, by decreasing the internal length scale, the model converges to the Griffith fracture; however, for any non-zero internal length scale damage, appears for any point of the material which has even an infinitesimal strain. 

Taking into account the internal length scale parameter as a material property has been motivated in~\cite{Pham2011,AMOR2009,Nguyen2016}, in order to make a connection between internal length scale and maximum tensile strength in~$1$-D case. Another approach to prevent damage in the points which doesn't have sufficient energy is to apply different thresholds see~\cite{Miehe2010a}.

\cite{PAGGI2017145}

\cite{BRYANT2018561}

\begin{equation}
  \label{elasticitytensor}
\mathbb{C}_0= \begin{bmatrix} \lambda+2\mu & \lambda & 0 \\ \lambda & \lambda+2\mu & 0 \\ 0&0& \mu
 \end{bmatrix}
\end{equation}



\subsection{Threshold for damage}
It is  pre-eminent to apply a threshold for damage to fulfill the following condition:
 \begin{equation}
  \label{ddot}
\dot{d}\geq0
  \end{equation}
The above condition states that damage can increase during time, and there is no healing in the material. To this end, 
several authors express their idea, for example, in~\cite{Bourdin2000} this condition fulfills by enforcing the irreversibility condition when the damage gets close to $1$:
 \begin{equation}
  \label{bourdinCR}
d(\bm{u},t>t_0) = 1~~~if ~d(\bm{u},t_0)\approx1
  \end{equation}
The preceding approach is not adequate, while dealing with a cohesive fracture or quasi-brittle fracture. Damage value ($d$) is directly connected to the bulk energy by damage driving force ($Y$); this leads to that in ~\cite{Miehe2010a}, they prevent from any decreasing in the driving force, and it is dealt as a history variable so it doesn't decrease during unloading:
 \begin{equation}
  \label{MieheCR}
Y\propto\psi_0^+=\mathcal{H}(\bm{u},t) := max ~\psi_0^+(\bm{u},t)
  \end{equation}
The same approach is adopted in the continuum damage models by~\cite{SIMO1987}.\\
 Introducing the damage criterion as $\mathcal{G}(\psi_0^+,d):=-{f_D}_c^{\prime}\psi_0^+-G_c\delta \gamma$ and having the energy conservation law, the Karush-Kuhn-Tucker conditions read as:
  \begin{equation}
  \label{kuhntucker}
\dot{d}\geq0,~~~~\mathcal{G}\leq 0,~~~~\mathcal{G}\dot{d}=0
  \end{equation}
The second condition reads :
  \begin{equation}
  \label{damageineq}
\int_\mathcal{B} \left[ {f_D}_c^{\prime}\left(d\right)\psi_0 \delta d + G_c \delta \gamma \right] dV \geq 0
  \end{equation} 
  in which 
    \begin{equation}
  \label{deltagamma}
\delta \gamma = \cfrac{1}{c_0}[\cfrac{1}{l_c}\alpha^{\prime}(d) \delta d + 2l_c \nabla d \cdot \nabla \delta d ]
  \end{equation} 
A more detailed explanation about the crack topology function $\alpha(d)$ and its characteristics can be found on appendix~\ref{AppendixB}. What is important here is that for regular phase-filed damage models with having $\alpha(d)=d^2$ the equation~\ref{damageineq} becomes a variational equality and naturally satisfied when $d(x)\in [0,1]$ see~\cite{BORDEN2012}. However, the existence of a linear term in crack topology might not satisfy the mentioned equation when $d(x)\in [0,1]$ see~\cite{wu2018}.
Another time looking back to gradient extended damage models see~\cite{FREMOND1996,Pham2011,MIEHE2011898}~and later in the PFMs see~\cite{Miehe2010a} reads the total energy potential as:
\begin{equation}
\label{potential}
W(\bm{u},d,\nabla d)=f_D\left(\psi_0 - \psi_{cs} \right) + \psi_{cs} + G_c \gamma(d,\nabla d)
 \end{equation} 
  Where $\psi_{cs}$ is the specific fracture energy per unit volume. Applying strain or stress thresholds, one can write the $\psi_{cs}$ for the $1$-D case as :
 \begin{equation}
\label{psics}
\psi_{cs}=~
\begin{cases}
 \cfrac{1}{2} E \epsilon_c^2 ~~\text{strain threshold damage starts when}~~ \epsilon \geq \epsilon_c \\
 \cfrac{\sigma_c^2}{2E} ~~~~~\text{strain threshold damage starts when}~~ \sigma \geq \sigma_c = t_0
\end{cases}
 \end{equation} 
In order to show why taking this approach is necessary, let us start with the Kuhn-Tucker condition another time and imagine damage wants to initiate, therefore,~$\dot{d}> 0$~and~ $d\approx 0$. Subsequently, the third condition of Kuhn-Tucker entails~$\mathcal{G}=0$. In order to simplify more the ${f_D}_c$ is substituted with~\ref{1_d2}, this simplification creates no problem since both functions converge to a negative number when $d\approx 0$.
\begin{equation}
\label{g0}
\mathcal{G}=-2(1-d)\psi_0^+-G_c\delta \gamma=0
 \end{equation} 
Inserting equation~\ref{deltagamma} into equation~\ref{g0} reads:
\begin{equation}
\label{g02}
\mathcal{G}=-2(1-d)\psi_0^++G_c\cfrac{1}{c_0}\left[\cfrac{1}{l_c}\alpha^{\prime}(d) \delta d + 2l_c \nabla d \cdot \nabla \delta d   \right] = 0
 \end{equation} 
During the initial steps of loading, this assumption is held $\psi_0^+\approx 0$; therefore, the later term in equation~\ref{g02} should fulfill the condition by itself. For regular crack topology function ($\alpha = d^2 )$ the condition is fulfilled when $d \approx 0 $, since the $ \alpha^{\prime}=d$ has been appeared and there is no need for threshold. However, for instance, taking into account $\alpha = 2d-d^2 )$  which reads as:
 \begin{equation}
\label{g03}
\mathcal{G}= \cfrac{G_c}{c_0}(2-2d) = 0,
 \end{equation} 
perfectly shows that damage wants to evolve almost at every single point ($d \Rightarrow 1$), without any need for sufficient bulk energy. \\
 This is why in~\cite{wu2020} a stress threshold has been implied according to ~\cite{Miehe2010a} as we have shown by equation~\ref{psics}. 
 By adding this term the following equation is obtained :
 \begin{equation}
\label{g04}
\mathcal{G}=-2(1-d)(psi_0^-\psi_{cs}) +\cfrac{G_c}{c_0}\left(\cfrac{1}{l_c} \left(2 -2d \right) + 2l_c \nabla d \cdot \nabla \delta d   \right) = 0
 \end{equation} 
 Finally, due to the value of $\psi_{cs}$ almost no damage is evolved before $\psi_0^+$ reaches a $\psi_{cs}$ in other words the initial value which is assigned to damage driving force $Y$ can compensate the effect of the linear term in the crack topology function. All in all, the complete procedure for applying threshold including loading and loading and also having different crack topology functions read as:
 \begin{equation}
  \label{thresholdhis}
Y\propto\psi_0^+=\mathcal{H}(\bm{u},t) := max\left(\cfrac{t_0^2}{2E},max ~\psi_0^+(\bm{u},t) \right)
  \end{equation}
  
  

Having defined the energy contributions in Eqs.~\ref{eq:ee_1} and \ref{eq:ec_1}, we apply the Euler-Lagrange approach (variational derivative) with respect to the displacement field $\boldsymbol{u}$ and the damage field $D$ on the total energy density function (i.e. $\psi = \psi^{ex}+\psi^{in}$). 

Moreover, the stress $\boldsymbol{\sigma}$ and damage driving force $Y$ are obtained in Eq.~\ref{eq:ee_2} and Eq.~\ref{eq:ee_3}, respectively.
\begin{align}
\label{eq:ee_2}
 \dfrac{\partial \psi_e}{\partial \boldsymbol{\epsilon}} &= \boldsymbol{\sigma} = \mathbb{C}:\boldsymbol{\epsilon} = f_D~\mathbb{C}_0 :\boldsymbol{\epsilon} + (1-f_D)~\mathbb{P}:\boldsymbol{\epsilon} ,\\
\label{eq:ee_3}
 \dfrac{\partial \psi_e}{\partial D} &= -Y = \dfrac{\text{d}f_D}{\text{d}D}~\underbrace{\dfrac{1}{2}~\boldsymbol{\epsilon}:\mathbb{C}_h:\boldsymbol{\epsilon}}_\text{$\psi^0_e$} = \dfrac{\text{d}f_D}{\text{d}D}~\psi^0_e.
\end{align}
The following relations are also stated here for later derivations:
\begin{align}
\label{eq:ec_3}
 \dfrac{\partial \psi_c}{\partial D} &= g_c~\dfrac{\partial \gamma}{\partial D} = g_c~\dfrac{D}{l_c},\\
\label{eq:ec_4}
 \dfrac{\partial \psi_c}{\partial \nabla D} &= g_c~\dfrac{\partial \gamma}{\partial \nabla D} + \gamma~\underbrace{\dfrac{\partial g_c}{\partial \nabla D}}_\text{$\boldsymbol{g}_d$} = g_c~l_c~\nabla D + \gamma~\boldsymbol{g}_d.
\end{align}

Considering the set of Eqs.~\ref{eq:ee_1}-\ref{eq:ee_3}, one obtains the main partial differential equations for the displacement field which are basically the same as the balance of linear momentum:
\begin{equation}
\label{eq:pde_1}
\delta_{\boldsymbol{u}} \psi = \partial_{\boldsymbol{u}} \psi - \text{div}(\partial_{\nabla \boldsymbol{u}} \psi) \Rightarrow  \left\{
\begin{array}{l}
    \text{div}(\boldsymbol{\sigma})+\boldsymbol{b} = \boldsymbol{0}~~~\text{in}~\Omega
\end{array}
\right.
\end{equation}


Considering Eqs.~\ref{eq:ec_1}-\ref{eq:ec_4}, one obtains the following equations for the damage field:
\begin{equation}
\label{eq:pde_2}
\delta_{D} \psi = \partial_{D} \psi - \text{div}(\partial_{\nabla D} \psi) \Rightarrow  \left\{
\begin{array}{l}
    \dfrac{g_c}{l_c}D - \text{div}(l_c~g_c \nabla D)- \text{div}(\gamma~\boldsymbol{g}_d) - Y_{m} = 0~~~\text{in}~\Omega
\end{array}
\right.
\end{equation} 

Here (as mentioned in Eq.~\ref{eq:ec_4}) we have $\boldsymbol{g}_d = \partial g_c / \partial \nabla D$. Furthermore, the so-called history variable field $Y_{m}$ is introduced to ensure the irreversibility condition upon unloading (see \cite{MIEHE20102765}). As defined below, the latter term is obtained via the maximum value of the stored undamaged elastic energy during the simulation time, i.e. $H={\text{max}}
(\psi^0_e(t))$. See also Eq.~\ref{eq:ee_3}. Therefore, the maximum damage driving force $Y_m$ in Eq.~\ref{eq:pde_2} is written as
\begin{align}
\label{eq:hist}
-Y_{m} = \dfrac{\text{d}f_D}{\text{d}D}~\underset{t}{\text{max}}(\psi^0_e(t)) =
\dfrac{\text{d}f_D}{\text{d}D}~H
\end{align}

Comparing Eq.~\ref{eq:pde_2} to the standard isotropic phase-field damage models one notice the following extensions: First, a new term, i.e. $\text{div}(\gamma~\boldsymbol{g}_d)$, is introduced. Second, the fracture energy is not constant anymore and is strongly coupled to the damage variable $D$. When $g_c$ is constant, then $\boldsymbol{g}_d = \partial g_c / \partial \nabla D \rightarrow \boldsymbol{0}$. In this case, the standard formulation is recovered.


%%%%%%%%%%%%%%%%
\subsection{Structural Tensor}
In this subsection, due to the work of~\cite{Teichtmeister17}, with the help of a second-order tensor~$\bm{A}$ the new form of a crack density function is written as:

\begin{equation}  
\label{anisoCr}
\gamma (d,\nabla {d},\bm{A})~=~\frac{1}{2l_c}d^2~+~\frac{l_c}{2} ~\nabla {d}. \bm{A}.\nabla {d} .
\end{equation}

By the coordinate-free representation of quadratic crack surface density functions, the structural tensor has the following feature
\begin{equation}  
\label{Asymm}
\bm{A}_{ij}~=~\bm{A}_{ji}.
\end{equation}

Since the symmetry of $\bm{A}$ second-order tensor, the anisotropic microstructure of the material is invariant, concerning the rotations of the symmetric group \cite{Teichtmeister17}.

Where~$\bm{a}$~ is a given structural direction with~$||\bm{a}||~=~1$. By means of $\bm{a}$~the following second-order structural tensor can be defined as:

\begin{equation}  
\label{2ndOmega}
\bm{\omega}:= \bm{a}~\otimes~\bm{a},
\end{equation}

Therefore,~ $\bm{A}$~is calculated as:
\begin{equation}  
\label{Aomg}
\bm{A}:= \bm{I}~+~\alpha \bm{\omega},
\end{equation}

Consequently, the anisotropy is computed by means~$\alpha$,~which is only a scalar parameter that weights the material direction. So on the isotropic metric tensor ~$\bm{I}$,~ is replaced by the anisotropic tensor~$\bm{A}$.

Orthonormal basis can be determined by the above structural directions~$\{\bm{a}_i\}_{i~=~1,2,3}$, hence the following relation holds:

\begin{equation}  
\label{orthonormalrelation}
\bm{a_i}~.~\bm{a_j}~=~\delta_{ij}~ and~\bm{a_i}~\times~\bm{a_j}~=~\epsilon_{ijk} ~\bm{a_k}
\end{equation}
Where~$\epsilon_{ijk}$~ is the Levi-Civita operator. So it reads the second-order structural tensors:
\begin{equation}  
\label{w12}
\bm{\omega_1}:= \bm{a_1}~\otimes~\bm{a_1}~~and~~\bm{\omega_2}:= \bm{a_2}~\otimes~\bm{a_2}
\end{equation}
reads:
\begin{equation}  
\label{A12tensors}
\bm{A_1}:= \bm{I}~+~\alpha_1 \bm{\omega_1}~~~ and~~~\bm{A_2}:= \bm{I}~+~\alpha_2 \bm{\omega_2}
\end{equation}
Representation of~$\omega$ in matrix notation can be written as:
\begin{equation}  
\label{wmatrix}
\bm{\underline{\omega}}= \begin{bmatrix}
\cos\left(\phi\right) & \cos\left(\phi\right) \sin\left(\phi\right) \\
cos\left(\phi\right) \sin\left(\phi\right) &\cos\left(\phi\right)
\end{bmatrix}
\end{equation}

After making the structural tensor for anisotropic damage, it is worth to mention that the internal length scale also gets affected by this tensor. In~\cite{Teichtmeister17}, the effective length scale is derived as :
\begin{equation}  
\label{efflc}
l^*_c=l_c\left(1+\alpha\cos^2\left(\phi-\theta\right)\right) 
\end{equation}
Considering~\ref{efflc} if the cracks follow the predefined path~$\left(\phi=\theta\right)$ the effective length scale will be:
\begin{equation}  
\label{efflcfollows}
l^*_c=l_c\left(1+\alpha\right) 
\end{equation}
The above relation plays a vital role for the simulation of the coating system, and defining the internal length scale~($l_c$)~ value, should be done by considering the above relation.
With having variational principles of~\ref{eulervariationpf}, the Euler equations can be rewritten as:
\begin{equation}  
\label{elerAtensorboun}
d-l^2_c~div \left(\bm{A}\nabla d\right)=0~~\text{in}~  \mathcal{B}~~\text{and,}~\left(\bm{A}\nabla d\right)\cdot \bm{n}=0~~\text{on}~~\partial \mathcal{B}
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%
\subsection{Arbitrary anisotropy}
Motivated by atomistic analysis of some materials, there is a necessity to introduce a function by which arbitrary shapes of anisotropy can be achieved. In this section, the formulation which is available in~\cite{Shahed20} is presented.

An approvable crack direction is determined by the shape of fracture energy: hence, the crack chooses a path in which the fracture energy is minimum. However, it is mentionable that the loading direction and boundary conditions have effects on the crack path, and deviation is feasible when the fracture energy difference for different directions, is not big enough.  \\
With taking into account
sharp crack direction as~$\bm{e_c}$~, crack is diffused by the variable ~$d(x)$~ ,see~figure~\ref{dx_diffuse}, The crack spreads out perpendicular to the direction~$\bm{e_c}$~see figure~\ref{fig:ecgdd} .$(\bm{e_c}~\perp~\nabla {d})$. \\
For formulating the direction-dependent fracture energy~$G_c(\theta)$~and entering it into the phase-field damage the~$\theta$~ can be written by damage gradient~$\nabla {d}$. By considering the gradient of damage,~$\phi$, the directional dependent fracture energy reads as:
  \begin{equation}
  \label{gcthea}
\begin{cases}
      \bm{e_c}~\perp~\nabla {d}~\Rightarrow~\theta~=~\phi - \pi / 2\\
     \phi~=~atan ~({(\nabla {d}~.~\bm{e_2})}/({\nabla {d}~.~\bm{e_1}}))\\
    \end{cases} 
    \Rightarrow~G_c(\theta)~=~g_c(\nabla d)
  \end{equation}
With introducing energy frequency functions as:
  \begin{equation}
  \label{emthet}
E_m(\theta)~=~\beta_m\left(1+\alpha_m\sin^2\left(\theta+\theta^{\prime}\right)\right)
  \end{equation}
  and sum of which over certain frequencies, one can get an arbitrary fracture energy function as:
   \begin{equation}
  \label{gcem}
G_c(\theta)=g_c(\nabla d)=G_c\sum_m E_m(\theta), ~m\in \mathbf{N}
  \end{equation}
The effect of this function on the weak form and implementation into the finite element method is discussed in the chapter~\ref{Chapter4}.


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Insesnsitive phase-field formulation using energetic and crack topology functions}
It has been noted that the global response of regular phase-field models is heavily dependent on the internal length scale parameter~($l_c$).
A group of researchers of the opinion that the internal length scale is a material parameter and via equation~\ref{lct0}, see~\cite{Miehe2010a,borden2011}. This parameter can be determined by considering the maximum tensile strength as:
 \begin{equation}
  \label{lct0}
t_0=\cfrac{9}{16}~\sqrt{\cfrac{EG_c}{3l_c}}
  \end{equation}
The equation~\ref{lct0} is often considered as a cohesive strength for a phase-field damage model in $1$-D. Hence, one can fit the parameter internal length scale~($l_c$) to get them an appropriate cohesive strength.
Because of this thesis's goal, which is predicting cracks for hard coatings, the internal length scale~($l_c$) should be considered as a numerical tool by which the crack zone and crack area can be controlled. Consequently the mesh independency can be achieved. Referring to the equation~\ref{efflc}~and~\ref{efflcfollows}, it can be interpreted that for the high anisotropic behavior cases one cannot fix the internal length scale~($l_c$) parameter to the desired value and it can heavily change the response. \\



0
Considering the equation~\ref{VintW}, the damage driving force now is introduced as~$Y$, which can be interpreted as a bridge that connects the stored energy of the bulk to the fracture energy. \\
With the regular type of degradation function~\ref{1_d2}, the damage driving force reads as:
\begin{equation}
  \label{ysimple}
Y=-2\left(1-d\right) \cfrac{1}{2} \bm{\epsilon^T}:\mathbb{C}_0:\bm{\epsilon}
  \end{equation}
The above equation reads as:
\begin{equation}
  \label{yfdl}
Y=-{f_D}^{\prime}_L \cfrac{1}{2} \bm{\epsilon^T}:\mathbb{C}_0:\bm{\epsilon}
  \end{equation}
Where the equation for~${f_D}^{\prime}_L$. 
Meanwhile, it is worthy to mention that localization is done between neighboring material points through a ~$\nabla^2 d$~into the yield function in gradient extended damage models, which is not the desire of this thesis. However, it should be mention that the final formulation for gradient extended damage models and phase-field damage models are almost sharing the same equations. 


According to Fig.~\ref{fig:body}, for a pure mechanical system, the external energy can be wirtten in terms of the external traction $\bm{t}^{ex}$ acting on $\Gamma_t$ as well as the body force vector $\bm{b}$ acting on the whole voluem. \textcolor{red}{think about gammat}
\begin{equation}
  \label{externalenergy}
 %\psi^{ex}(\bm{u},\bm{b},\bm{t}^{ex})=\bm{b} \cdot \bm{u} + %\bm{t}^{ex} \cdot \bm{u}.
 \psi^{ex}(\bm{u},\bm{b})=\bm{b} \cdot \bm{u}.
\end{equation}

\Psi=\int_{\Omega} \psi~dV = \int_{\Omega} \psi^{ex}(\bm{u},\bm{b})~dV + \int_{\Gamma_t}t_{ex}~dA +

\begin{equation}
 \label{totalenergy}
 \Psi=\int_{\Omega} \psi~dV = 
 \int_{\Omega} \psi_e(\nabla \bm{u},d)~dV + \int_{\Gamma_c} \psi_c(d,\nabla d)~dA.
\end{equation}

\begin{equation}
    \psi_c=G_c A_c
\end{equation}
Thanks to the phase field formulation and introducing crack density function we can transfer the surface integral to the volume integral.
\begin{equation}
\label{psiC}
    \psi_c=G_c \gamma(d,\nabla d)
\end{equation}

%%%%%%%%%% TAKEN FROmFRMULATION
%In the numerical example part, we have shown that despite the global response of the system is independent of the internal length scale, the crack path is differed heavily from the preferred direction. Teichtmeister \cite{Teichtmeister17} has shown the effective length-scale as 
%\begin{equation}
%    \label{efflength}
%    l_c^*=l_c(1+\alpha \sin^2(\theta+\phi))
%\end{equation}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Fig2.jpg}
    \caption{comparing the crack paths of CPF, SPF and CZM models (for the isotropic damage case)}
    \label{fig:Figure2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/Fig3.jpg}
    \caption{comparing the response of CPF, SPF and CZM models (for the isotropic damage case)}
    \label{fig:Figure3}
\end{figure}

%\textbf{Remark 2.} For the case with arbitrary anisotropy, the maximum value of the fracture energy is $G_c(1+\alpha)$. By taking a similar approach one can easily obtain the relations defined in Eq.~\ref{a1_araniso}. Motivated by the work of \cite{HOSSAIN2018118}, one can also consider an anisotropic distribution for the maximum tensile strength ($t_0$).


%Applying the threshold enables us to have an initial linear stage for stress.

%According to~\cite{MIEHE2015449} we another time reintroduce a threshold as:

%Previously in \cite{Shahed21}, the arbitrary model is used for the standard phase-field damage model. With having the narrower band for damage, insensitive formulation cannot predict the crack path without any other further assumption.

%Reconsideration of equation~\ref{thresholdeq1} the similar approach is considered for the threshold so we have following thresholds for two variants of anisotropy.
%\begin{align}
%\label{ThFdFunctions}
%\psi_{th,s}=\dfrac{1}{2E}t_0^2,~~~ 
%\psi_{th,a}=\dfrac{1}{2E}t_d^2
%\end{align}



%\delta \bm{u}=\bm{N}_u \delta \bm{u}_e \\
% \delta d = \bm{N}_d \delta d_e
% \nabla \delta d = \bm{B}_d \delta d_e

The penalizing damage is the base for the structural tensor method. Due to the narrower damage zone in insensitive formulation, this issue can be problematic when it comes to the anisotropic fracture energy for initially isotropic materials.



%%%%%%%%%%%%%% before algoo %%%%%%%%%%%
Utilizing a stagger approach, the stiffness matrix for a single element is derived as follows, where only the off-diagonal terms are considered. 
\begin{equation}
\label{Kstag}
\bm{K}_e=
\begin{bmatrix}
 {\left[\bm{K}_{uu}\right]_{8\times8}} & {\left[\bm{0}\right]}_{4\times8} \\ {\left[\bm{0}\right]}_{8\times4} &{\left[\bm{K}_{dd}\right]}_{4\times4}
\end{bmatrix}_{12\times12}.
\end{equation}
Note that due to the non-convexity of minimization problem with respect to the damage and displacement field, using the staggered approach leads to the more robust algorithm \cite{MIEHE201027}.
The essential terms in matrix \ref{Kstag} read as:
\begin{equation}
\label{Kuu}
{\bm{K}_{uu}}=\dfrac{\partial  \bm{r}_u}{\partial \bm{u}_e} =  \left[\int_{\mathcal{B}}  \bm{B}^T_u \bm{C}(d) \bm{B}_u ~dV\right]_{8\times8},
\end{equation}

\begin{equation}
\label{Kdd,s}
{\bm{K}_{dd,s}} =\dfrac{\partial  \bm{r}_d}{\partial d_e} =  \int_{\mathcal{B}} \left[  \dfrac{2l_cG_c}{\pi}\bm{B}^T_d \bm{A}\bm{B}_d +  \bm{N}^T_d \left( {f_D}^{\prime \prime}H + \dfrac{\omega^{\prime \prime}(d) G_c}{\pi l_c}\right) \bm{N}_d \right]_{4\times4} dV.
\end{equation} 

\begin{equation}
\label{Kdd,a}
{\bm{K}_{dd,a}} =\dfrac{\partial  \bm{r}_d}{\partial d_e} =  \int_{\mathcal{B}} \left[  \dfrac{2l_c g_c^n (\nabla d)}{\pi}\bm{B}^T_d \bm{B}_d +  \bm{N}^T_d \left( {f_D}^{\prime \prime}H + \dfrac{\omega^{\prime \prime}(d) g_c^n (\nabla d)}{\pi l_c}\right) \bm{N}_d \right]_{4\times4}dV.
\end{equation} 

It noteworthy that increasing this value could results in convergence problem and increases the number of iteration. \textcolor{red}{what value?}
According to~\cite{REZAEI2021a}, an explicit scheme is used for determining the $\theta$ by means of $\nabla d$. For further details one can refer to the mentioned details. The following conditions have been used for the model. \textcolor{red}{we should redo the last paragraph}

\begin{equation}
\label{conditionfor_directional}
\begin{cases}
d \leq 0.1 \to \begin{cases} g_c(\nabla d)=G_c (1+\alpha) \\
t_0(\theta)=t_0 \end{cases}\\
 0.1< d \leq 0.95 \to  \begin{cases} g_c(\nabla d)=G_c(1~+~\alpha \sin^2(m(\theta+\phi))) \\
t_0(\theta)=t_0(1~+~\alpha \sin^2(m(\theta+\phi)))^n\end{cases}\\
d>0.95 \to \begin{cases} g_c(\nabla d)=G_c \\
t_0(\theta)=t_0 \end{cases}
\end{cases}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Solving the system with a monolithic approach, enforces us to compute all the terms. However, with using the staggered solvers, only $2$~components of upper stiffness matrix are needed.
% For the case of arbitrary anisotropy the later term changes to :
%%%%%%%%%%%%%%

%\subsection{Staggered algorithm}
%Due to the non-convexity of related free-energy with respect to %both fields, which is appeared for the monolithic approach see~\cite{GERASIMOV2016276}, the robust but slow rate convergence achieved. it is common to use the staggered approach. \\

%By decoupling the stiffness matrix to the relevant damage and displacement parts, and solving each part, while the other part has been frozen, a faster and equally accurate approach accomplished; this method is called "staggered". 
%So instead of the following system of equations:
%\begin{equation}
%\label{mmosys}
%\begin{bmatrix}
 %{\left[\bm{K}_{uu}\right]}_{8\times8} & %{\left[\bm{K}_{ud}\right]}_{8\times4}\\
 %{\left[\bm{K}_{du}\right]}_{4\times8} & %{\left[\bm{K}_{dd}\right]}_{4\times4}
%\end{bmatrix}_{12\times12} 
%\begin{bmatrix}
 %{\left[\bm{U}_{\bm{u}_e}\right]}_{8\times1}\\
% {\left[\bm{U}_{d_e}\right]}_{4\times1}
%\end{bmatrix}_{12\times1}
%=
%\begin{bmatrix}
% {\left[\bm{r}_u\right]}_{8\times1}\\
% {\left[\bm{r}_d\right]}_{4\times1}
%\end{bmatrix}_{12\times1}
%\end{equation}
%Two systems of equations are solving for each iteration; therefore, one additional iteration is needed; nonetheless, the effect of smaller matrix size can compensate for this effect and delivers a faster convergence with having no convexity problem.
%\begin{equation}
%\begin{cases}
%{\left[\bm{K}_{uu}\right]}_{8\times8}{\left[\bm{U}_{\bm{u}_e}\right]}_{8\times1}= {\left[\bm{r}_u\right]}_{8\times1}\\
%\text{The above equation has been soler for the new iteration $i+1$} \\
%\text{with having the $d_i$ value from the previous iteration} \\
%\text{then with having the $\bm{U}_{i+1}$ values the other system solve} \\
%{\left[\bm{K}_{dd}\right]}_{4\times4}~{\left[\bm{U}_{d_e}\right]}_{4\times1}= {\left[\bm{r}_d\right]}_{4\times1}\\
%\text{and finally, the value for $d_{i+1}$ is computed} 
%\end{cases}
%\end{equation}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/RFLvsS.jpg}
    \caption{comparing the response of CPF, SPF and CZM models (for the isotropic damage case) for geometries A and B. }
    \label{fig:RFLvsS}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/RFLvsS2.jpg}
    \caption{comparing the response of CPF, SPF and CZM models (for the isotropic damage case) for geometries A and B. }
    \label{fig:RFLvsS}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ali's explanations
The results of Fig.~\ref{fig:anisoSCPF} clearly indicated that the internal length-scale parameter has an influence on the crack path. The later observation is specifically bold for the anisotropic CPF formulation while is hardly detectable for the standard formulation.

In the work of Wu et al. \cite{wu2021} the anisotropic behavior is captured by the special form of helmholtz free energy for initially anisotropic fracture energy based on \cite{Gultekin2016}. \\

Based on the damage evolution Eq.~\ref{deltadsttensor}, we argue that $\dfrac{\partial \psi_c}{\partial \nabla d}$ should remain constant with the change of the internal-length scale to get an insensitive crack path.
so we have:
\begin{equation}
    \label{dgcdd}
    \dfrac{\partial \psi_c}{\partial \nabla d}  = \dfrac{2 G_c}{\pi}~l_c \alpha \bm{A} \cdot \nabla d
    %= \dfrac{2 G_c l_c}{\pi}~\alpha \bm{A} \cdot \nabla d \to
\end{equation}
In Figure \ref{fig:?}, it is shown that by decreasing the internal length scale parameter the $\alpha$ should be increased to get the same crack path.
A vital issue here is that the $\alpha$ increase will be result in the higher fracture energy in forbidden direction however one have to keep in mind that the process zone has the wide of $l_{ch}$ which is the characteristic length of cohesive zone models, despite the internal length scale parameter. This is why we suggest that for proper and real values of fracture energy values one should keep this length in mind and then go for taking the penalty parameter so we have:
\begin{equation}
    \label{gc_eff}
G_c^{eff} = (\alpha+1) l_{ch}/2 
\end{equation}
for proving the later point we have perform the test and prescribing the angle of crack. For two cases and investigate the effect of the identical penalty parameter $\alpha$ for different lengths.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Previous Appendix B 
\section{Appendix B: Equations for arbitrary anisotropy} 
Changing the value of fracture energy with respect to the gradient of damage ($G_c(\nabla d)$) is changing the eqution~\ref{ELd}.a. Hence, the equation should be rewritten, and a new form for discretization should be computed.
According to \cite{Shahed20} the Euler-Lagrange equation for damage can be rewritten as:
\begin{equation}
\label{eldAA}
\delta_{d}\psi =\dfrac{G_c}{\pi l_c} \left(2d-d^2\right) -div\left(\dfrac{l_c G_c}{c_0 \pi} \nabla d \right) -div\left(\gamma \bm{g}_d\right)- Y=0~\text{in}~ \mathcal{B} 
\end{equation}
Where~$\bm{g}_d= \partial G_c/\partial (\nabla d)$, and the derivation follows from a chain rule as:
\begin{equation}
\label{gdchain}    
\bm{g}_d=\dfrac{\partial G_c}{\partial (\nabla d)}= \dfrac{\partial G_c}{\partial \theta}\dfrac{\partial \theta}{\partial (\nabla d)}
\end{equation}
Where the first term can be computed easily, by having equation~\ref{gcem}~and~\ref{emthet}. Taking into consideration one of the frequency, this term reads as:
\begin{equation}
\label{dgcthet}
\dfrac{\partial G_c}{\partial \theta}= G_c\alpha_m \alpha_m \sin\left(2m(\theta+\theta^{\prime}) \right)
\end{equation}
In order to compute the other term firstly, the following figure has been plotted in order to show the relation between $\theta$ and $\nabla d$.
\begin{figure}[H]
    \centering
        \includegraphics[width=0.5\linewidth]{Figures/Figures_3/ecgdd.pdf}

    \caption{schematic representation of $\nabla d~ \text{and}~e_c $ }
    \label{fig:ecgdd}
\end{figure}
As it can be observed from the figure~\ref{fig:ecgdd}, the $\nabla d$ unit vector is perpendicular to the crack normal vector $e_c$, by taking this into consideration, one can obtain the following relation for the second term of equation~\ref{gdchain} as:
\begin{equation}
\label{gddthet}
\dfrac{\partial \theta}{\partial (\nabla d)}= \dfrac{1}{{|\nabla d|}^2} \begin{bmatrix}
 -{\nabla d}_y \\ ~{\nabla d}_x
\end{bmatrix}
\end{equation}
Going back to equation~\ref{eldAA}, and considering the $\bm{g}_d$ derivation, one can get the discretization formulation follows as:
\begin{equation}
\label{weakgd}
\int_\mathcal{B} \underbrace{\left(\bm{d}_e^T \bm{N}^T_d\right)}_{u} \underbrace{\left( div(\gamma \bm{g}_d )\right)}_{v^{\prime}} dV 
\end{equation}
Performing an integration by parts rule for the equation~\ref{weakgd}, reads:
\begin{equation}
\label{weakgd1}
\bm{d}_e^T \bm{N}^T \gamma \bm{g}_d \Big|_{\Gamma_c} - \int_\mathcal{B} \bm{d}_e^T \bm{B}_d^T \gamma \bm{g}_d dV
\end{equation}
Having equation~\ref{ELd}.c and the value of damage at damage around crack $d=0$ the first term of equation~\ref{weakgd1} equals to zero. So to summarize the equation and compute the extra term in the weak form with considering arbitrary anisotropy, the combination of~\ref{weakgd1},~\ref{gddthet}, and~\ref{dgcthet} reads for the first of $\gamma$:
\begin{equation}
\label{extraterm}
\int_\mathcal{B} \bm{B}_d^T \dfrac{\alpha(d)}{c_0\pi} \bm{g}_d dV=  \dfrac{\partial G_c}{\partial \theta} \dfrac{\alpha(d)}{c_0\pi} \int_\mathcal{B}    \bm{d}_e^T\underbrace{\left(2 \bm{N}\bm{d}_e - \bm{d}_e^T\bm{d}_e    \right) \bm{B}_d^T \begin{bmatrix}
 -{\nabla d}_y \\ ~{\nabla d}_x
\end{bmatrix}}_{\bm{a}}
\end{equation}

Simplification can be made here for $\bm{a}$:
\begin{equation}
\label{asimple}
\bm{a}=\left(2\bm{N}-\bm{d}_e^T\right)\bm{d}_e \bm{B}_d^T \begin{bmatrix}
 -{\nabla d}_y \\ ~{\nabla d}_x
\end{bmatrix}=\bm{a}=\left(2\bm{N}-\bm{d}_e^T\right)
\underbrace{
\begin{bmatrix}
 {\nabla d}_x & ~{\nabla d}_y
\end{bmatrix}\begin{bmatrix}
 -{\nabla d}_y \\ ~{\nabla d}_x
\end{bmatrix}}_{\bm{b}}
\end{equation}
Finally $\bm{b}$ reads as :
\begin{equation}
\label{bsimple}
\bm{b}=-{\nabla d}_x{\nabla d}_y+{\nabla d}_x{\nabla d}_y = \underbar{0}
\end{equation}
The second term of $\gamma$ which is also dependent of $\nabla d$ reads as:
\begin{equation}
\label{staa1}
\dfrac{\partial G_c}{\partial \theta}~\dfrac{\alpha(d)}{c_0\pi} \int_\mathcal{B}   \dfrac{1}{{|\nabla d|}^2} \bm{B}^T\begin{bmatrix}
 -{\nabla d}_y \\ ~{\nabla d}_x 
 \end{bmatrix}\bm{d}_e\bm{B}_d^T \bm{B}_d \bm{d}_e^T
\end{equation}
Like the previous simplification, the preceding equation reads as:
\begin{equation}
\label{staa2}
\dfrac{\partial G_c}{\partial \theta}~\dfrac{\alpha(d)}{c_0\pi} \int_\mathcal{B}    \bm{B}^T\underbrace{\dfrac{1}{{|\nabla d|}^2}\begin{bmatrix}
 -{\nabla d}_y \\ ~{\nabla d}_x 
 \end{bmatrix} \begin{bmatrix}
{\nabla d}_x & {\nabla d}_y 
 \end{bmatrix}}_{\bm{C}}\bm{B}_d \bm{d}_e^T 
\end{equation}
$\bm{C}$ can be rewritten as:
\begin{equation}
\label{c2nd}
\bm{C}=\dfrac{1}{{|\nabla d|}^2}\begin{bmatrix}
 -{\nabla d}_y \\ {\nabla d}_x
 \end{bmatrix} \begin{bmatrix}
{\nabla d}_x & {\nabla d}_y 
 \end{bmatrix}=\dfrac{1}{{|\nabla d|}^2}\begin{bmatrix}
  -{\nabla d}_y {\nabla d}_x & -{\nabla d}_y {\nabla d}_y \\ {\nabla d}_x {\nabla d}_x & {\nabla d}_y {\nabla d}_x
  \end{bmatrix}
\end{equation}
Considering the following relations:
\begin{equation}
\label{cossin}
\theta = \tan^{-1} \dfrac{{-\nabla d}_x}{{\nabla d}_y}, ~~~~\sin(\theta)=\dfrac{{\nabla d}_x}{{|\nabla d|}^2}, ~~~~\cos(\theta)=\dfrac{{-\nabla d}_y}{{|\nabla d|}^2},
\end{equation} 

The latest form of $\bm{c}$ has the following form:
\begin{equation}
\label{c2ndorder}
 \bm{C}=\begin{bmatrix}
\sin(\theta)\cos(\theta)  &  -\cos(\theta)\cos(\theta) \\
\sin(\theta)\sin(\theta) &-\sin(\theta)\cos(\theta)
 \end{bmatrix}   
\end{equation}

The above second-order tensor $\bm{C}$ is similar to the structural tensor it has been introduced in chapter~\ref{Chapter2}.
%%
%%previous algo all in 1
\begin{algorithm}[H]
\label{alg:algo_directional}
\SetAlgoLined 
 initialize the damage value (in order to find the crack direction $\theta$): \textcolor{red}{why do we need this?} \\ %$d^{i+1}=d^i$
 $d^i$: damage value of Gauss points from the previous time step\\
 \While{Newton iteration to solve for $u^{i+1} \text{and}~d^{i+1}$ \textcolor{red}{we should need another index}}{
 $\nabla d^i =\bm{B}_d \bm{d}_e^i$ \\
  \eIf{$||\nabla d^i|| \ge ||\nabla d_c||$}{
   $\theta^{i} =tan^{-1} \left( \dfrac{\nabla d^i_y}{\nabla d^i_x} \right)$ \\
   $\sigma_{u}^{i} = \sigma_{u,0}(1 + \alpha \sin^2(m(\theta^i+\phi)))^{pm}$\\
    $g_c^{i} = G_{c,0}(1 + \alpha \sin^2(m(\theta^i+\phi)))$
   }{
   $\sigma_{u}^{i}=\sigma_u$\\
   $g_c^i=G_{c,0}(1+\alpha)$
  
  }
  update the arbitrary threshold and degradation function
   $\psi_{th}^{i}=\dfrac{1}{2E}\sigma_{u}^{i}$ \\
  $a^i_{1}=\dfrac{4 E G_{c,0} (1+\alpha)}{\pi l_c ~(\sigma^i_{u})^2}$\\
   Newton iteration for displacement field\\
\While{${\bm{u}_{e,k+1}^{i+1}}-{\bm{u}_{e,k}^{i+1}} \leq tol$}{${\bm{r}_{u,k+1}^{i+1}}=-  \int_{\Omega} \left(\bm{B}^T_u \bm{C}(d^i) \bm{B}_u {\bm{u}_{e,k+1}^{i+1}} - \bm{N}^T_u \bm{b}  \right) dV - \int_{\partial \Gamma_t} \bm{N}^T_u \bm{t}~dA$\\
  ${\bm{K}_{uu,k+1}^{i+1}}= \int_{\mathcal{B}}  \bm{B}^T_u \bm{C}(d^i) \bm{B}_u ~dV$ \\
  $\Delta \bm{u}^{i+1}_{e,k+1}= \bm{u}_{e,k+1}^{i+1}- \bm{u}_{e}^{i+1}=\bm{K}^{i+1}_{uu,k+1} \bm{r}_{u,k+1}^{i+1}$\\
$k=k+1$
} 
  $H^{i}= \max_t (\psi_e^{i+1}(t), \psi^{i}_{th}) $\\ Newton iteration for damage field\\
  \While{${\bm{d}_{e,k+1}^{i+1}}-{\bm{d}_{e,k}^{i+1}} \leq tol $}{\\
  $f_D = \dfrac{(1-\bm{d}_{e,k+1})^2}{(1-\bm{d}_{e,k+1})^2+a_1^{i}\bm{d}_{e,k+1}+a_1^i a_2\bm{d}_{e,k+1}^2}$\\
  \textcolor{blue}{we should talk hwo to explain this degradation function}\\
  ${\bm{r}_{d,k+1}^{i+1}}=-\int_{\Omega} \left(\dfrac{2 g_c^{i} l_c}{\pi} \bm{B}^T_d \bm{B}_d {\bm{d}_{e,k+1}^{i+1}} +\bm{N}^T_d\left(\dfrac{\omega^{\prime}({\bm{d}_{e,k+1}^{i+1}}) g_c^{i}}{c_0l_c} - f_D^{\prime}(\bm{d}_{e,k+1}^{i+1})H^i \right)\right) dV$ \\
  ${\bm{K}_{dd,k+1}^{i+1}} =\int_{\mathcal{B}} \left( \dfrac{2l_c g_c^{i}}{\pi}\bm{B}^T_d \bm{B}_d +  \bm{N}^T_d \left( {f_D}^{\prime \prime}(\bm{d}_{e,k+1}^{i+1})H^{i} + \dfrac{\omega^{\prime \prime}({\bm{d}_{e,k+1}^{i+1}}) g_c^{i} }{\pi l_c}\right) \bm{N} \right)dV$\\
$\Delta \bm{d}^{i+1}_{e,k+1}= \bm{d}_{e,k+1}^{i+1}- \bm{d}_{e,k}^{i+1}=\bm{K}^{i+1}_{dd,k+1} \bm{r}_{d,k+1}^{i+1}$\\
$k=k+1$
 }
 update the undamaged tensile elastic stored energy:\\
 $\psi_e^{i+1}(t)=\dfrac{1}{2}\bm{\epsilon}:\mathbb{C}:\bm{\epsilon}$
 }
 \caption{Semi-implicit staggered scheme to solve the anisotropic PF fracture model}
\end{algorithm}


\begin{equation} %(\theta,||\nabla d||_c)
  \label{gcdef}
G_{c,\theta} = \begin{cases}
G_{c,max},~~~~~~~~~~~~~~~\text{if}~~~||\nabla d|| < ||\nabla d||_c\\
G_c(\theta)=g_c(\nabla d),~~~\text{if}~~~||\nabla d|| \geq ||\nabla d||_c
\end{cases}
\end{equation}








\begin{algorithm}[H]
\label{alg:ArMainAlgo}
\SetAlgoLined 
\caption{Staggered algorithm for the case of arbitrary anisotropy}
Inputs: ~~$\bm{d}_e^i$~~\,and  $\bm{u}_e^i$ \\ 
Outputs: $\bm{d}_e^{i+1}$~and  $\bm{u}_e^{i+1}$ \\
\\
Calculate $\sigma_{u}^{i}$ and $g_{c}^{i}$ via Alg.~\ref{alg:ArExplicit} \\
update the threshold for damage and degradation function constants \\
   $\psi_{th}^{i}=\dfrac{1}{2E}\sigma_{u}^{i}$ \\ \\
  $a^i_{1}=\dfrac{4 E G_{c,0} (1+\alpha)}{\pi l_c ~(\sigma^i_{u})^2}$\\
first part of the staggered solver (displacement field) call \ref{alg:DispStagg}\\
second part of the staggered solver (damage field) call 
\ref{alg:DamageStagg} \\
\end{algorithm}

\begin{algorithm}[H]
\label{alg:ArExplicit}
\SetAlgoLined 
  \caption{Computation of directional fracture energy and maximum tensile strength}
inputs: ~~$\bm{d}_e^i$, $\nabla d_c$, and pm\\ 
outputs: $g_c^i$~and~$\sigma_{u}^{i}$ \\
\\
computing element damage gradient\\
 $\nabla d^i =\bm{B}_d \bm{d}_e^i$ \\
  \eIf{$||\nabla d^i|| \ge ||\nabla d_c||$}{
   $\theta^{i} =tan^{-1} \left( \dfrac{\nabla d^i_y}{\nabla d^i_x} \right)$ \\
   $\sigma_{u}^{i} = \sigma_{u,0}(1 + \alpha \sin^2(m(\theta^i+\phi)))^{\text{pm}}$\\
    $g_c^{i} = G_{c,0}(1 + \alpha \sin^2(m(\theta^i+\phi)))$
   }{
   $\sigma_{u}^{i}=\sigma_u$\\
   $g_c^i=G_{c,0}(1+\alpha)$
  }
\end{algorithm}

\begin{algorithm}[H]
\label{alg:DispStagg}
\SetAlgoLined 
  \caption{Staggered solver for the displacement field}
inputs: ~~$\bm{u}_e^i$ and $\psi_{th}^i$\\ 
outputs: $\bm{u}_e^{i+1}$ and $H^i$ \\
   Newton iteration solving the differential equation for displacement field\\
\While{${\bm{u}_{e,k+1}^{i+1}}-{\bm{u}_{e,k}^{i+1}} \leq tol$}{${\bm{r}_{u,k+1}^{i+1}}=-  \int_{\Omega} \left(\bm{B}^T_u \bm{C}(d^i) \bm{B}_u {\bm{u}_{e,k+1}^{i+1}} - \bm{N}^T_u \bm{b}  \right) dV - \int_{\partial \Gamma_t} \bm{N}^T_u \bm{t}~dA$\\
  ${\bm{K}_{uu,k+1}^{i+1}}= \int_{\mathcal{B}}  \bm{B}^T_u \bm{C}(d^i) \bm{B}_u ~dV$ \\
  $\Delta \bm{u}^{i+1}_{e,k+1}= \bm{u}_{e,k+1}^{i+1}- \bm{u}_{e}^{i+1}=\bm{K}^{i+1}_{uu,k+1} \bm{r}_{u,k+1}^{i+1}$\\
$k=k+1$
}
 update the undamaged tensile elastic stored energy:\\
 $\psi_e^{i+1}(t)=\dfrac{1}{2}\bm{\epsilon}:\mathbb{C}:\bm{\epsilon}$\\
 updating the history value for exporting to the damage solving part\\
 $H^{i}= \max_t (\psi_e^{i+1}(t), \psi^{i}_{th})$
\end{algorithm}

\begin{algorithm}[H]
\label{alg:DamageStagg}
\SetAlgoLined
inputs: ~~$\bm{d}_e^i$, $g_c^i$, $\sigma_u^i$ and $H^i$\\ 
outputs: $\bm{d}_e^{i+1}$\\
 \caption{Staggered solver for the damage part}
  \While{${\bm{d}_{e,k+1}^{i+1}}-{\bm{d}_{e,k}^{i+1}} \leq tol $}{\\

  ${\bm{r}_{d,k+1}^{i+1}}=-\int_{\Omega} \left(\dfrac{2 g_c^{i} l_c}{\pi} \bm{B}^T_d \bm{B}_d {\bm{d}_{e,k+1}^{i+1}} +\bm{N}^T_d\left(\dfrac{\omega^{\prime}({\bm{d}_{e,k+1}^{i+1}}) g_c^{i}}{c_0l_c} - f_D^{\prime}(\bm{d}_{e,k+1}^{i+1})H^i \right)\right) dV$ \\
  ${\bm{K}_{dd,k+1}^{i+1}} =\int_{\mathcal{B}} \left( \dfrac{2l_c g_c^{i}}{\pi}\bm{B}^T_d \bm{B}_d +  \bm{N}^T_d \left( {f_D}^{\prime \prime}(\bm{d}_{e,k+1}^{i+1})H^{i} + \dfrac{\omega^{\prime \prime}({\bm{d}_{e,k+1}^{i+1}}) g_c^{i} }{\pi l_c}\right) \bm{N} \right)dV$\\
$\Delta \bm{d}^{i+1}_{e,k+1}= \bm{d}_{e,k+1}^{i+1}- \bm{d}_{e,k}^{i+1}=\bm{K}^{i+1}_{dd,k+1} \bm{r}_{d,k+1}^{i+1}$\\
$k=k+1$
 }

\end{algorithm}

\begin{algorithm}[H]
\label{alg:ArMainAlgo}
\SetAlgoLined 
\caption{Staggered algorithm for the case of arbitrary anisotropy}
Inputs: ~~$\bm{d}_e^i$, $\bm{u}_e^i$, $||\nabla d_c||$ and material properties \\ 
Outputs: $\bm{d}_e^{i+1}$~and  $\bm{u}_e^{i+1}$ \\

 $\nabla d^i =\bm{B}_d \bm{d}_e^i$ $\to$    $\theta^{i} =tan^{-1} \left( \dfrac{\nabla d^i_y}{\nabla d^i_x} \right)$\\
  \eIf{$||\nabla d^i|| \ge ||\nabla d_c||$}{
   Compute $g_c^{i}$ via Eq. \ref{gc_theta}\\
   Compute $\sigma_{u}^{i}$ via Eq. \ref{sigma_u_theta}
   }{
   Set $g_c^i = G_{c,max}$ \\
   Set $\sigma_{u}^{i} = \sigma_0$ 
  }
Update $\psi_{th}^{i}$ via Eq.~\ref{H1} \\
Update $a^i_{1}$ via Eq.~\ref{a1_araniso}\\

call~Algorithm~$2$\\
call~Algorithm~$3$
\end{algorithm}



\begin{algorithm}[H]
\label{alg:DispStagg}
\SetAlgoLined 
\caption{Staggered solver for the displacement field}
Inputs: ~~$\bm{u}_e^i$ and $\psi_{th}^i$\\ 
Outputs: $\bm{u}_e^{i+1}$ and $H^i$ \\ \\
Newton solver for displacement field (Eq.~\ref{ru})\\
\While{${\bm{u}_{e,k+1}^{i+1}}-{\bm{u}_{e,k}^{i+1}} \leq tol$}{${\bm{r}_{u,k+1}^{i+1}}=-  \int_{\Omega} \left(\bm{B}^T_u \bm{C}(d^i) \bm{B}_u {\bm{u}_{e,k+1}^{i+1}} - \bm{N}^T_u \bm{b}  \right) dV - \int_{\partial \Gamma_t} \bm{N}^T_u \bm{t}~dA$\\
  ${\bm{K}_{uu,k+1}^{i+1}}= \int_{\mathcal{B}}  \bm{B}^T_u \bm{C}(d^i) \bm{B}_u ~dV$ \\
  $\Delta \bm{u}^{i+1}_{e,k+1}= \bm{u}_{e,k+1}^{i+1}- \bm{u}_{e}^{i+1}= (\bm{K}^{i+1}_{uu,k+1})^{-1}~ \bm{r}_{u,k+1}^{i+1}$\\
$k=k+1$
} 
Update $\psi_e^{i+1}=\dfrac{1}{2}\bm{\epsilon}^{i+1}:\mathbb{C}^i:\bm{\epsilon}^{i+1}$ \\
Update $H^{i}= \max (\psi_e^{i+1}, \psi^{i}_{th})$  
\end{algorithm}





\begin{algorithm}[H]
\label{alg:DamageStagg}
\SetAlgoLined
\caption{Staggered solver for the damage field}
Inputs: ~~$\bm{d}_e^i$, $g_c^i$, $\sigma_u^i$ and $H^i$\\ 
Outputs: $\bm{d}_e^{i+1}$\\ \\
Newton solver for the damage field (Eq.~\ref{rda})\\
  \While{${\bm{d}_{e,k+1}^{i+1}}-{\bm{d}_{e,k}^{i+1}} \leq tol $}{\\
  ${\bm{r}_{d,k+1}^{i+1}}=-\int_{\Omega} \left(\dfrac{2 g_c^{i} l_c}{\pi} \bm{B}^T_d \bm{B}_d {\bm{d}_{e,k+1}^{i+1}} +\bm{N}^T_d\left(\dfrac{\omega^{\prime}({\bm{d}_{e,k+1}^{i+1}}) g_c^{i}}{c_0l_c} - f_D^{\prime}(\bm{d}_{e,k+1}^{i+1})H^i \right)\right) dV$ \\
  ${\bm{K}_{dd,k+1}^{i+1}} =\int_{\mathcal{B}} \left( \dfrac{2l_c g_c^{i}}{\pi}\bm{B}^T_d \bm{B}_d +  \bm{N}^T_d \left( f_D^{\prime \prime}(\bm{d}_{e,k+1}^{i+1})H^{i} + \dfrac{\omega^{\prime \prime}({\bm{d}_{e,k+1}^{i+1}}) g_c^{i} }{\pi l_c}\right) \bm{N} \right)dV$\\
$\Delta \bm{d}^{i+1}_{e,k+1}= \bm{d}_{e,k+1}^{i+1}- \bm{d}_{e,k}^{i+1} = (\bm{K}^{i+1}_{dd,k+1})^{-1}~ \bm{r}_{d,k+1}^{i+1}$\\
$k=k+1$
 }
\end{algorithm}


%It reads the equation~\ref{eulervariationpf} when the crack is completed as:
%\begin{equation}  
%\label{condialfa}
%\begin{cases}
%\omega^{\prime}-2l_c^2~ \Delta d =0~~~~ in~~ B\\
%\nabla d \cdot n =0~~~~~~~~~~on ~~\partial B
%\end{cases}
%\end{equation}

%\begin{figure}[H]
%\label{cracktopog}
%\centering
%\includegraphics[width=0.5\linewidth]{Figures/cracktopolog.jpg} %{a}
%\caption{crack ultimate phase-field~$d_u$ for different crack topology function}
%\end{figure}
%\appendix 


\begin{align}  
\begin{split}
\label{psicAa}
\psi_{c,a} &= \dfrac{G_{c,0}}{c_0l_c} ~\left(\omega(d)~+~l_c^2~\nabla d^T \, \bm{A} \, \nabla d  \right) \\
&=\dfrac{G_{c,0}}{c_0l_c} ~\left(\omega(d)~+~\alpha~l_c^2~\nabla d^T \, \begin{bmatrix}
c^2(\phi) & c(\phi)s(\phi)\\
c(\phi)s(\phi) & s^2(\phi)
\end{bmatrix} ||\nabla d||^2 \, \nabla d  ~+~l_c^2 \nabla d^T \nabla d \right) \\
& \text{with having the Eq. \ref{theta} the direction of $\nablda d$ can be represented by~$\beta=\left( \dfrac{\nabla d \cdot e_2}{\nabla d \cdot e_1} \right)=\theta +\pi/2$} \\
& \text{Finally one gets: $\nabla d = \begin{bmatrix} c(\beta) \\ s(\beta)
\end{bmatrix}$} \\
&=\dfrac{G_{c,0}}{c_0l_c} ~\left(\omega(d)~+~\alpha~l_c^2~\begin{bmatrix} c(\beta)& s(\beta)  \end{bmatrix}~\begin{bmatrix} c^2(\phi)\,c(\beta)\,+\,c(\phi)\,c(\beta)\,s(\beta) \\ c(\phi)\,s(\phi)\,c(\beta)\,+s^2(\phi)\,s(\beta) \end{bmatrix}||\nabla d||^2 \,+\,l_c^2 \nabla d^T \nabla d \right) \\
&=\dfrac{G_{c,0}}{c_0l_c} ~\left(\omega(d)~+~\alpha~l_c^2~\left(c(\phi)c(\beta)+s(\phi)s(\beta)  \right)^2 \,+\,l_c^2 \nabla d^T \nabla d \right) \\
&=\dfrac{G_{c,0}}{c_0l_c} ~\left(\omega(d)~+~\alpha~l_c^2~\cos^2(\beta-\phi)||\nabla d||^2 \,+\,l_c^2 \nabla d^T \nabla d \right) \\
&=\text{by reconsidering $\beta\,=\,\theta\,+\,\pi/2$}, \text{this leads to}: \\
&=\dfrac{G_{c,0}}{c_0l_c} ~\left(\omega(d)~+~\left(1\,+\,\alpha~l_c^2~\sin^2(\theta-\phi)\right)||\nabla d||^2\right)
\end{split}
\end{align}

%\textcolor{red}{lets add $0.04~l_c$ later.}
%\textcolor{blue}{if you mean for the small one we cannot since we end up with fully broken state and nonsense result but we can mention that maybe in a text}
%to set this parameter as $0.04~l_c$.

 %\While{$||{\bm{u}_{e,k+1}^{i+1}}-{\bm{u}_{e,k}^{i+1}}|| \leq tol$}

 %According to studies in \cite{REZAEI2021a}, the scalar parameter $||\nabla d_c||$ is a numerical parameter which has to be adjusted depending on the problem. 
 
 \begin{align}
\label{fdd}
\bm{g}_d &=\dfrac{\partial g_c}{\partial \nabla d} =  \dfrac{\partial g_c}{\partial \theta}~\dfrac{\partial \theta}{\partial \nabla d}, \\
\bm{s}_d &=\dfrac{\partial f_D}{\partial \nabla d} =  \dfrac{\partial f_D}{\partial a_1}~\dfrac{\partial a_1}{\partial \theta}~\dfrac{\partial \theta}{\partial \nabla d}
\end{align}
